Investigating transformers in the decomposition of polygonal shapes as point collections

Transformers can generate predictions in two approaches: 1. auto-regressively by conditioning each sequence element on the previous ones, or 2. directly produce an output sequences in parallel. While research has mostly explored upon this difference on sequential tasks in NLP, we study the difference between auto-regressive and parallel prediction on visual set prediction tasks, and in particular on polygonal shapes in images because polygons are representative of numerous types of objects, such as buildings or obstacles for aerial vehicles. This is challenging for deep learning architectures as a polygon can consist of a varying carnality of points. We provide evidence on the importance of natural orders for Transformers, and show the benefit of decomposing complex polygons into collections of points in an auto-regressive manner.

==> sections/method_experiments_Jan.tex <==
\section{Method}
\andrea{I have just written this and the following sections, they are not part of my paper yet}.
To study upon the difference between conditional vs joint probability, I have developed 4 models. They are alla based on DETR, which is shown in figure \ref{fig:DETR}.
\subsection{DETR for Gates: \emph{joint probability}}
This is basically DETR in which I modified one of the last FFNs to output 4 points instead of a bounding box (DETR was used originally for simple object detection). So instead of a final tensor of dimension 4 $[x_{c}, y_{c}, height, width]$, I output a tensor of dimension 8 $[x_{1}, y_{1}, x_{2}, y_{2}, x_{3}, y_{3}, x_{4}, y_{4},]$.
Its Transformer Decoder starts with 100 \emph{object queries} and each of them is classified into the GATE class or the NO-OBJECT class. Each object query can look at all other queries in the attention layer, because there is no masking. 
    
\subsection{DETR auto-regressive for Gates: \emph{conditional probability}}
This model changes the Transformer Decoder module of DETR drastically. Instead of using 100 object queries, we use sentences of tokens. There are 3 possible tokens in our vocabulary: \emph{start}, \emph{gate} and \emph{end-of-computation}. If we want to train the model on an image which contains 3 gates, the sentence will be
\[s, g, g, g, eoc\]
This sentence is generated one-token-by-one, by passing all the previous tokens at the bottom of the decoder to generate the next one.
    
\subsection{DETR with RNN: \emph{joint probability}}
This architecture is used to predict \emph{polygons} and is similar to \textbf{DETR for gates}. The difference is at the end of the architecture. In \textbf{DETR for gates}, we pass each object query (a vector of dimension 256) through a FFN that outputs a vector of dimension 8 $[x_{1}, y_{1}, x_{2}, y_{2}, x_{3}, y_{3}, x_{4}, y_{4},]$. Here, instead of this FFN, we have a simple RNN that takes each object query independently and outputs N points, followed by a STOP signal that ends the recurrence. Equally to \textbf{DETR for gates}, the object queries are all visible in the attention layer (no masking), thus modelling the joint probability.


\subsection{DETR auto-regressive for polygons: \emph{conditional probability}}
This is equal to \textbf{DETR auto-regressive for Gates}, but needs to work with polygons. The vocabulary is now \emph{start}, \emph{point}, \emph{end-of-polygon} and \emph{end-of-computation}. The sentence is once again generated auto-regressively. If we want to train the model on an image which contains 2 polygons, one of 3 corners and one of 4 corners, the sentence will be:
\[s, p, p, p, eop, p, p, p, p, eop, eoc\]


\section{Experiments}
We test these models on four datasets. Two of them are an instance of a \emph{set prediction problem} and two of them are an instance of a \emph{double set prediction problem.}
\begin{itemize}
    \item \textbf{Toy setting for gates}: as shown in figure \ref{toy_gate}, these are black \& white, generated images of polygons of 4 corners.
    \item \textbf{Real gates}: as shown in figure \ref{real_gate}, these are images of real gates in the scenario of a flying UAV.
    \item \textbf{Toy setting for polygons}: as shown in figure \ref{toy_poly}, these are black \& white, generated images of polygons of $N$ corners.
    \item \textbf{CrowdAI}: as shown in figure \ref{real_poly}, these are satellite images of buildings. The task is to draw the outer shape of each building.
\end{itemize}

The results are shown in table \ref{results_datasets}. From these results we can conclude different things.
First we confirm that on gate detection, our models outperform a strong baseline such as Mask R-CNN. Then, we show that \textbf{for regular \emph{set prediction problems}, modeling the joint probability of our variables is more effective}. This is because the attention layer without any masking is allowed to compare \textbf{all} of its inputs against each other, which is a great help when all elements of the set can be represented in the same way (all gates have 4 corners). On the other hand, when moving to a \emph{double set prediction problem} such as the polygon detection, the elements of the set are all different (polygons have different amounts of corners) and the global computation of the attention layer is not an important factor any more. Instead, dividing the large problem of polygon detection into smaller problems of detecting one point by one, becomes the best solution and the conditional probability beats the joint one by more than 20\% absolute mAP. This is because each element of the chain of conditional probabilities lives in a smaller space which turns out to be easier to model.

In table \ref{results_order} we report the averaged results of the study on the imposed order of the auto-regressive solutions and of the addition of artificial positional encodings to the Transformer decoder. We show that the imposed order has a great effect on the performance of the model even when there is no natural order in what we are trying to model (set of polygons in an image) and that manually adding information about the position of previously generated tokens actually undermines the performance of the model. In short, \emph{what} was previously generated is a lot more important than \emph{the order} in which it was done.

\clearpage
